Learn the Task, Not the Schedule: Reducing Spurious Cross-Arm Coupling in Bimanual Imitation Learning

A bimanual demonstration specifies both what the robot should do and one particular schedule for when each arm should act. Standard imitation learning does not distinguish task-required cross-arm constraints from incidental scheduling choices, and may therefore exploit opposite-arm progress as a shortcut cue, creating spurious cross-arm coupling even where relative timing is irrelevant for the current task phase. We introduce Constraint-preserving Temporal Recombination (CTR), a training-time data intervention that preserves recorded arm-local sensorimotor content while retiming the corresponding segments to realize admissible schedules that preserve task-required cross-arm constraints. We use CTR to train Diffusion Policy, Action Chunking with Transformers, and $\pi_{0.5}$, and evaluate them on four simulated and four real-robot tasks. Across six real-robot bimanual progress-state initializations, CTR raises worst-state success from 56% for the strongest non-CTR schedule mixture to 76%. With $\pi_{0.5}$ on an Independent task, a 4 s pause transfers 2.56 s of delay to the opposite arm under the Concurrent schedule distribution, but only 0.25 s with CTR. On real robots, CTR violates task constraints in only 0--4% of trials, versus 36--98% for narrow-schedule baselines. Code will be released at https://github.com/MINT-SJTU/CTR.

==> tables/pause_duration_full.tex <==
\begin{tabular}{llccccc}
\toprule
Model & Data & 1\,s & 2\,s & 3\,s & 4\,s & $\beta_{\rm delay}\downarrow$ \\
\midrule
\multirow{4}{*}{DP} & $L\!\rightarrow\!R$ & 0.95 / 85 & 1.87 / 79 & 2.79 / 72 & 3.71 / 66 & 0.92 \\
 & Concurrent & 0.81 / 87 & 1.60 / 82 & 2.39 / 77 & 3.18 / 72 & 0.79 \\
 & Mixed & 0.44 / 92 & 0.87 / 89 & 1.30 / 86 & 1.73 / 84 & 0.43 \\
 & CTR & 0.17 / 96 & 0.30 / 95 & 0.43 / 94 & 0.56 / 93 & 0.13 \\
\midrule
\multirow{4}{*}{ACT} & $L\!\rightarrow\!R$ & 0.91 / 87 & 1.80 / 81 & 2.69 / 75 & 3.58 / 69 & 0.89 \\
 & Concurrent & 0.78 / 89 & 1.55 / 84 & 2.32 / 79 & 3.09 / 74 & 0.77 \\
 & Mixed & 0.40 / 94 & 0.79 / 91 & 1.18 / 88 & 1.57 / 86 & 0.39 \\
 & CTR & 0.14 / 97 & 0.24 / 96 & 0.34 / 96 & 0.44 / 95 & 0.10 \\
\midrule
\multirow{3}{*}{$\pi_{0.5}$} & $L\!\rightarrow\!R$ & 1.33 / 60 & 2.82 / 66 & 3.78 / 90 & 5.12 / 56 & 1.232 \\
 & Concurrent & 0.54 / 72 & 1.48 / 64 & 3.00 / 72 & 2.56 / 58 & 0.758 \\
 & CTR & 0.44 / 86 & 0.27 / 100 & 0.40 / 100 & 0.25 / 100 & -0.042 \\
\bottomrule
\end{tabular}


==> tables/pause_duration_main.tex <==
\AddToHookNext{env/tabular/begin}{\color{black}}
\begin{tabular}{lc!{\hspace{2pt}}c!{\hspace{2pt}}c!{\hspace{2pt}}cc}
\toprule
Data & 1\,s & 2\,s & 3\,s & 4\,s & $\beta_{\rm delay}\downarrow$ \\
\midrule
$L\!\rightarrow\!R$ & 1.33 / 60 & 2.82 / 66 & 3.78 / 90 & 5.12 / 56 & 1.232 \\
Concurrent & 0.54 / 72 & 1.48 / 64 & 3.00 / 72 & 2.56 / 58 & 0.758 \\
CTR & 0.44 / 86 & 0.27 / 100 & 0.40 / 100 & 0.25 / 100 & -0.042 \\
\bottomrule
\end{tabular}


==> tables/pause_summary_full.tex <==
\begin{tabular}{llrrr}
\toprule
Model & Data & $\beta_{\rm delay}\downarrow$ & $\Delta T_{\rm other}(4\,{\rm s})\downarrow$ & $\mathrm{SR}_{\rm other}(4\,{\rm s})\uparrow$ \\
\midrule
\multirow{4}{*}{DP} & $L\!\rightarrow\!R$ & 0.92 & 3.71 & 66 \\
 & Concurrent & 0.79 & 3.18 & 72 \\
 & Mixed & 0.43 & 1.73 & 84 \\
 & CTR & 0.13 & 0.56 & 93 \\
\midrule
\multirow{4}{*}{ACT} & $L\!\rightarrow\!R$ & 0.89 & 3.58 & 69 \\
 & Concurrent & 0.77 & 3.09 & 74 \\
 & Mixed & 0.39 & 1.57 & 86 \\
 & CTR & 0.10 & 0.44 & 95 \\
\midrule
\multirow{3}{*}{$\pi_{0.5}$} & $L\!\rightarrow\!R$ & 1.232 & 5.12 & 56 \\
 & Concurrent & 0.758 & 2.56 & 58 \\
 & CTR & -0.042 & 0.25 & 100 \\
\bottomrule
\end{tabular}

